Improved Robustness to Open Set Inputs via Tempered Mixup

Supervised classification methods often assume that evaluation data is drawn from the same distribution as training data and that all classes are present for training. However, real-world classifiers must handle inputs that are far from the training distribution including samples from unknown classes. Open set robustness refers to the ability to properly label samples from previously unseen categories as novel and avoid high-confidence, incorrect predictions. Existing approaches have focused on either novel inference methods, unique training architectures, or supplementing the training data with additional background samples. Here, we propose a simple regularization technique easily applied to existing convolutional neural network architectures that improves open set robustness without a background dataset. Our method achieves state-of-the-art results on open set classification baselines and easily scales to large-scale open set classification problems.

==> mixup_comp.tex <==
% \begin{table}[]
% \centering
% \caption{\textbf\{Tempered Mixup comparison to Mixup\} AUOSC scores for classification of either MNIST or CIFAR-10 as known classes and various unknown classes.  For both known datasets the benefit of both Mixup and Tempered Mixup over baseline confidence thresholding is most substantial as the unknown dataset becomes more similar to the known classes.  Additionally for the most similar unknown datasets, Tempered Mixup provides a clear benefit in open-set performance over standard Mixup augmentation.}
% \label{tab:mixup_comp}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}rcccccc@{}}
% \toprule
% \textit{Known} & \textit{MNIST} & \textit{MNIST} & \textit{MNIST} & \textit{CIFAR} & \textit{CIFAR} & \textit{CIFAR} \\ \midrule
% \multicolumn{1}{r|}{\textit{Unknown}} & \textit{Gaussian Noise} & \textit{Fashion MNIST} & \textit{EMNIST-Letters} & \textit{SVHN} & \textit{LSUN} & \textit{TinyImageNet} \\ \midrule
% \multicolumn{1}{r|}{\textit{Baseline}} & \textbf{0.9878} & 0.9848 & 0.9066 & 0.8271 & 0.7934 & 0.7694 \\
% \multicolumn{1}{r|}{\textit{Mixup}} & 0.9874 & \textbf{0.9875} & 0.9737 & 0.8193 & 0.7966 & 0.7886 \\
% \textit{Tempered Mixup} & 0.9846 & \textbf{0.9875} & \textbf{0.9821} & \textbf{0.8340} & \textbf{0.8062} & \textbf{0.8099} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{\textsc{Tempered Mixup comparison to Mixup} AUOSC scores for classification of either MNIST or CIFAR-10 as known classes and various unknown classes.  For both known datasets the benefit of both Mixup and Tempered Mixup over baseline confidence thresholding is most substantial as the unknown dataset becomes more similar to the known classes.  Additionally for the most similar unknown datasets, Tempered Mixup provides a clear benefit in open-set performance over standard Mixup augmentation.}
\label{tab:mixup_comp}
\resizebox{\textwidth}{!}{%
\begin{tabular}{r|cccccc}
\hline
\textit{Known} & \textit{MNIST} & \textit{MNIST} & \textit{MNIST} & \textit{CIFAR} & \textit{CIFAR} & \textit{CIFAR} \\ \hline
\textit{Unknown} & \textit{Gaussian Noise} & \textit{Fashion MNIST} & \textit{EMNIST-Letters} & \textit{SVHN} & \textit{LSUN} & \textit{TinyImageNet} \\ \hline
\textit{Baseline} & \textbf{0.9878} & 0.9848 & 0.9066 & 0.8271 & 0.7934 & 0.7694 \\
\textit{Mixup} & 0.9874 & \textbf{0.9875} & 0.9737 & 0.8193 & 0.7966 & 0.7886 \\
\textit{Tempered Mixup} & 0.9846 & \textbf{0.9875} & \textbf{0.9821} & \textbf{0.8340} & \textbf{0.8062} & \textbf{0.8099} \\ \hline
\end{tabular}%
}
\end{table}
